Annotation-free Learning of Deep Representations for Word Spotting using Synthetic Data and Self Labeling

Word spotting is a popular tool for supporting the first exploration of historic, handwritten document collections. Today, the best performing methods rely on machine learning techniques, which require a high amount of annotated training material. As training data is usually not available in the application scenario, annotation-free methods aim at solving the retrieval task without representative training samples. In this work, we present an annotation-free method that still employs machine learning techniques and therefore outperforms other learning-free approaches. The weakly supervised training scheme relies on a lexicon, that does not need to precisely fit the dataset. In combination with a confidence based selection of pseudo-labeled training samples, we achieve state-of-the-art query-by-example performances. Furthermore, our method allows to perform query-by-string, which is usually not the case for other annotation-free methods.

==> gfx/standalone_iterative/color-config.tex <==
% Farbpaletten fuer das TU Dortmund Cooperate Design.
% Leitfarbe jeder Palette ist jeweils das TU gruen.

\definecolor{tucol1}{rgb}{1.0 0.5 0.05}
\definecolor{tucol2}{rgb}{0.52,0.72,0.10}
\definecolor{tucol3}{rgb}{0.0 0.0 0.8}
\definecolor{tucol5}{rgb}{0.8 0.8 0}
\definecolor{tucol4}{rgb}{0.8 0 0.8}
\definecolor{tucol6}{rgb}{0 0.8 0.8}


% kraeftig
\definecolor{tucol-kraeftig1}{RGB}{132,184,25}
\definecolor{tucol-kraeftig2}{RGB}{216,148,39}
\definecolor{tucol-kraeftig3}{RGB}{27,161,175}
\definecolor{tucol-kraeftig4}{RGB}{168,0,135}
\definecolor{tucol-kraeftig5}{RGB}{239,228,32}
\definecolor{tucol-kraeftig6}{RGB}{202,116,40}

% kuehl
\definecolor{tucol-kuehl1}{RGB}{132,184,25}
\definecolor{tucol-kuehl2}{RGB}{233,238,168}
\definecolor{tucol-kuehl3}{RGB}{217,233,229}
\definecolor{tucol-kuehl4}{RGB}{191,218,187}
\definecolor{tucol-kuehl5}{RGB}{113,176,96}
\definecolor{tucol-kuehl6}{RGB}{211,223,99}

% warm
\definecolor{tucol-warm1}{RGB}{132,184,25}
\definecolor{tucol-warm2}{RGB}{112,61,46}
\definecolor{tucol-warm3}{RGB}{193,178,40}
\definecolor{tucol-warm4}{RGB}{228,200,38}
\definecolor{tucol-warm5}{RGB}{178,175,132}
\definecolor{tucol-warm6}{RGB}{165,134,83}

% Rottoene
\definecolor{tucol-rot1}{RGB}{132,184,25}
\definecolor{tucol-rot2}{RGB}{196,21,58}
\definecolor{tucol-rot3}{RGB}{157,19,42}
\definecolor{tucol-rot4}{RGB}{119,24,40}
\definecolor{tucol-rot5}{RGB}{97,126,31}
\definecolor{tucol-rot6}{RGB}{58,82,11}

% Gruentoene
\definecolor{tucol-gruen1}{RGB}{132,184,25}
\definecolor{tucol-gruen2}{RGB}{214,223,42}
\definecolor{tucol-gruen3}{RGB}{97,134,39}
\definecolor{tucol-gruen4}{RGB}{148,164,33}
\definecolor{tucol-gruen5}{RGB}{182,201,48}
\definecolor{tucol-gruen6}{RGB}{115,158,64}

% Blautoene
\definecolor{tucol-blau1}{RGB}{132,184,25}
\definecolor{tucol-blau2}{RGB}{11,161,226}
\definecolor{tucol-blau3}{RGB}{36,123,196}
\definecolor{tucol-blau4}{RGB}{40,140,141}
\definecolor{tucol-blau5}{RGB}{177,213,230}
\definecolor{tucol-blau6}{RGB}{13,75,127}


==> gfx/standalone_iterative/tikz-config.tex <==

\usetikzlibrary{arrows,arrows.meta}
\usetikzlibrary{positioning,shapes,shapes.geometric,automata,fit,calc,decorations.pathreplacing,angles,quotes,backgrounds}
\usepgfplotslibrary{external}
%\tikzexternalize[prefix=gfx/Images-TikZ/]
\tikzset{%
%	every picture/.style={yscale=-1},
	every loop/.style={in=50,out=130,looseness=3},
	every node/.style={thin, font=\small},
	>=stealth
}

